Operationalizing Complex Causes: A Pragmatic View of Mediation

We examine the problem of causal response estimation for complex objects (e.g., text, images, genomics). In this setting, classical \emph{atomic} interventions are often not available (e.g., changes to characters, pixels, DNA base-pairs). Instead, we only have access to indirect or \emph{crude} interventions (e.g., enrolling in a writing program, modifying a scene, applying a gene therapy). In this work, we formalize this problem and provide an initial solution. Given a collection of candidate mediators, we propose (a) a two-step method for predicting the causal responses of crude interventions; and (b) a testing procedure to identify mediators of crude interventions. We demonstrate, on a range of simulated and real-world-inspired examples, that our approach allows us to efficiently estimate the effect of crude interventions with limited data from new treatment regimes.

==> sections/proofs.tex <==
% \section{Proofs}
% \label{sec:proofs}


% \begin{lemma}
% If $W \indep Y~|~Z^\star \cup \{X\}$, then there exists some scalar $\phi_X(Z^\star)$ such that $W \indep Y~|~\{\phi_X( Z^\star), X\}$.
% \end{lemma}

% \paragraph{Proof.} We will discuss the case for binary $Y$, as the proof for linear-Gaussian models follows the same idea. Let the structural equation for $Y$ be given by $f_y(x, \pi_Z, \pi_U)$, where $\pi_Z$ and $\pi_U$ are the observed and unobserved parents of $Y$ in the corresponding causal graph. The conditional distribution of $Y$ is given by
% \begin{align}
% p(y~|~x, \mathbf z^\star) = \nonumber\\
% p(f_y(x, \pi_Z, \pi_U) = 1~|~x, \mathbf z^\star)^y \times \nonumber\\
% (1 - p(f_y(x, \pi_Z, \pi_U) = 1~|~x, \mathbf z^\star))^{1 - y}.
% \nonumber
% \end{align}
% By assumption, $f_y(\cdot)$ is functionally independent of $W$. Now we just have to show that the random variable $f_y(x, \pi_Z, \pi_U)$ is conditionally independent of $W$ given $X$ and $Z^\star$. Since $W \indep Y~|~Z^\star \cup \{X\}$, it cannot be the case that $W$ and $\pi_{\backslash Z^\star, X}$, the parents of $Y$ not in $Z^\star \cup \{X\}$, are conditionally dependent given $Z^\star \cup \{X\}$. We define $\phi_X(\mathbf z^\star)$ as $p(f_y(x, \pi_Z, \pi_U) = 1~|~x, \mathbf z^\star)$ for each possible realization of $X$. Given $X$, we can fully reconstruct from $\phi_X(\mathbf z^\star)$ a conditional distribution of $Y$ that makes information about $W$ irrelevant. $\Box$




% \begin{theorem}
%   If $W \nindep Y~|~Z^\star \cup \{X\}$, and
  
%   \[
%     \displaystyle
%     \sum_{\mathbf{z}^\star \in \Phi_{x\mathbf{z}^\star}^f}p(y~|~w, x, \mathbf{z}^\star)\frac{p(\mathbf{z}^\star~|~w, x)}{\mathrm{Pr}(Z^\star \in \Phi_{x\mathbf{z}^\star}^f~|~w, x)} \neq
%   \]
%   \begin{equation}    
%     \sum_{\mathbf{z}^\star \in \Phi_{x\mathbf{z}^\star}^f}p(y~|~x, \mathbf{z}^\star)\frac{p(\mathbf{z}^\star~|~x)}
%     {\mathrm{Pr}(Z^\star \in \Phi_{x\mathbf{z}^\star}^f~|~x)},
%   \label{eq:lemma1}
%   \end{equation}

%   \noindent for some value $f$ in the range of $\phi_x(\cdot)$, then $W \nindep Y~|~\{\phi_X( Z^*), X\}$.
% \nonumber
% \end{theorem}

% %\begin{proof}[\textbf{\emph{Proof of Lemma~\ref{lemma:1}}}]
% \paragraph{Proof.} 
% Assume, contrary to the hypothesis, that $W \indep Y~|~\{ \phi_X(Z^\star), X\}$. Then
% \[
%   p(y~|~w, x, \phi_x(Z^\star) = f) = p(y~|~x, \phi_x(Z^\star) = f) \Rightarrow
% \]
% \[
%   \sum_{\mathbf{z}^\star} p(y~|~w, x, \phi_x(Z^\star) = f, \mathbf z^*)p(\mathbf{z}^*~|~w, x, \phi_x(Z^\star) = f) = 
% \]
% \[
%   \sum_{\mathbf{z}^\star} p(y~|~x, \phi_x(Z^\star) = f, \mathbf z^\star)p(\mathbf{z}^\star~|~x, \phi_x(Z^\star) = f) \Rightarrow
% \]
% \[
%   \sum_{\mathbf{z}^\star} p(y~|~w, x, \mathbf{z}^\star)p(\mathbf{z}^\star~|~w, x, \phi_x(Z^\star) = f) = 
% \]
% \[
%   \sum_{\mathbf{z}^\star} p(y~|~x, \mathbf{z}^\star)p(\mathbf{z}^*~|~x, \phi_x(Z^\star) = f) \Rightarrow
% \]
% \[
%  \displaystyle
%  \sum_{\mathbf{z}^\star \in \Phi_{x\mathbf{z}^\star}^f}p(y~|~w, x, \mathbf{z}^\star)\frac{p(\mathbf{z}^\star~|~w, x)}
%  {\mathrm{Pr}(Z^\star \in \Phi_{x\mathbf{z}^\star}^f~|~w, x)} =
% \]
% \[
%  \displaystyle
%  \sum_{\mathbf{z}^\star \in \Phi_{x\mathbf{z}^\star}^f}p(y~|~x, \mathbf{z}^\star)\frac{p(\mathbf{z}^\star~|~x)}
%   {\mathrm{Pr}(Z^\star \in \Phi_{x\mathbf{z}^\star}^f~|~x)},  
% \]
% which contradicts the hypothesis. $\hfill\Box$

==> sections/related.tex <==

Our method combines elements of causal discovery (structure learning) and inference (effect estimation). The former has a long tradition, from parametric tests of conditional independence \citep{Spirtes2000} to more modern optimization-based approaches \citep{zheng_dags_tears}. Effect estimation typically assumes that the causal structure is (at least partially) known, and exploits this knowledge to compute causal estimands. Previous efforts to combine causal discovery and inference have been limited to input-output pairs \citep{gultchin20a}, and do not typically consider high-dimensional objects, as we do here.

A frequent target in causal inference is the conditional average treatment effect (CATE), which measures the expected change in potential outcomes between a pair of intervention values $w, w'$, conditional on a set of covariates $Z$. A number of authors in recent years have proposed two-step learning procedures for CATE estimation, with separate models for $\E[W~|~Z]$ and $\E[Y~|~Z]$ \citep{Chernozhukov2018, VanderLaan2018, Hahn2020}. Our procedure likewise breaks effect estimation down into modular components, but with different structural assumptions designed to identify causal mediators. Whereas two-step CATE estimators are commonly restricted to univariate, binary treatments, we make no such assumption in our setup. The more recent work of \cite{nabi2017} targets perfect interventions on a possibly high-dimensional treatment vector. We emphasize, however, that the goal of these methods, such as double-machine learning \citep{Chernozhukov2018}, is to attain statistical efficiency for CATE estimation under (measured) confounding. In our case, the goal is to provide methods for sharing parameters across regimes by exploiting a notion of mediation.

Our method bears some resemblance to algorithms that exploit environmental invariance \citep{arjovsky2020invariant, Buhlmann2020, peters2016}. We assume, as in the instrumental variables setting, that (i) there exists a causal path from the treatment (policy, environment, etc.) to the outcome through some intermediate variable(s), i.e. $W \rightarrow X \rightarrow Y$; and (ii) there exists no direct path from the treatment to the outcome, i.e. $W \indep Y~|~X$ (and perhaps some possible confounders $Z$). However, we differ from these methods by focusing on the estimand $p(y~|~do(w))$ as opposed to just detecting the parents of $Y$ or using $W$ as a means to achieve a more robust predictor for $\E[Y~|~X]$.

What we call \emph{crude} interventions are most similar to so-called \emph{uncertain}/\emph{unknown} interventions \citep{eaton2007exact,rothenhausler2015backshift,ke2019learning,jaber2020causal,brouillard2020differentiable}. Out of these, our work most resembles the setup of \citet{eaton2007exact} and \cite{jaber2020causal}, who derive structure learning algorithms to discover the targets of interventions. However, our work differs from these as we are primarily interested in directly predicting the (conditional) response under intervention without reporting the causal structure among the target variables of the interventions.

More fundamentally, a crude intervention may appear similar to the notion of \emph{soft}/\emph{imperfect} interventions \citep{eberhardt2007interventions,kocaoglu2019characterization,correa2020calculus,huang2020causal}. However, the analogy is inexact. Soft interventions have a stochastic effect at some fixed level of description (e.g., a policy that reduces smoking by 90\% instead of 100\%), but still assume there are targets that can in principle be precisely manipulated. By contrast, crude interventions assume the existence of (at least) two valid levels of description -- a micro-level at which data are observed, and a macro-level at which treatments are administered.

Our emphasis on variable granularity has roots in the causal abstraction literature \citep{Beckers2019}. Learning coarse-grained causal features \citep{chalupka2016unsupervised} or disentangled representations \citep{locatello19a} from observational data in an unsupervised manner is impossible without introducing some inductive bias. Rather than insisting on a purely data-driven approach, we observe that, in many real-world cases, domain knowledge can help guide the transition from lower to higher levels of abstraction. 


